Riemannian-Geometric Fingerprints of Generative Models

Recent breakthroughs and rapid integration of generative models (GMs) have sparked interest in the problem of model attribution and their fingerprints. For instance, service providers need reliable methods of authenticating their models to protect their IP, while users and law enforcement seek to verify the source of generated content for accountability and trust. In addition, a growing threat of model collapse is arising, as more model-generated data are being fed back into sources (e.g., YouTube) that are often harvested for training ("regurgitative training"), heightening the need to differentiate synthetic from human data. Yet, a gap still exists in understanding generative models' fingerprints, we believe, stemming from the lack of a formal framework that can define, represent, and analyze the fingerprints in a principled way. To address this gap, we take a geometric approach and propose a new definition of artifact and fingerprint of GMs using Riemannian geometry, which allows us to leverage the rich theory of differential geometry. Our new definition generalizes previous work (Song et al., 2024) to non-Euclidean manifolds by learning Riemannian metrics from data and replacing the Euclidean distances and nearest-neighbor search with geodesic distances and kNN-based Riemannian center of mass. We apply our theory to a new gradient-based algorithm for computing the fingerprints in practice. Results show that it is more effective in distinguishing a large array of GMs, spanning across 4 different datasets in 2 different resolutions (64 by 64, 256 by 256), 27 model architectures, and 2 modalities (Vision, Vision-Language). Using our proposed definition significantly improves the performance on model attribution, as well as a generalization to unseen datasets, model types, and modalities, suggesting its practical efficacy.

==> sec/00-tldr.tex <==
We provide a new definition of fingerprints of generative models that generalize to non-Euclidean data (e.g., images, texts) using Riemannian geometry and manifold learning.

==> sec/algo-1-learn-rmetric.tex <==
\algopullback



==> sec/algo-2-compute-rcm.tex <==
Intrinsic gradient descent algorithms on Riemannian manifolds are well-known algorithm (see e.g., \cite{absil2008optimization} or \cite{udricste2000geometric}).
In locating the center of mass of a set of data points, we are interested in the so-called intrinsic algorithms, \ie, algorithms that are independent of the parametrization of the manifold. One natural idea is to use geodesic descent, that is, at a point on the manifold move along the geodesic in the direction of the negative of the gradient of the cost function (see e.g., \cite{absil2008optimization} or \cite{udricste2000geometric}). We call such an algorithm a gradient descent algorithm.
For later reference we derive the intrinsic gradient descent algorithm for locating the Riemannian $L^{p}$ center of mass.
% (see \cite{AbsMahSep2008} or \cite{Udriste_Book} for introduction to optimization on Riemannian manifolds). 
% 
One can check that:
\begin{equation}\label{eq:grad_Lp}
\nabla f_{p}(x)=-\sum_{i=1}^{N} w_{i}d^{p-2}(x,x_{i})\exp_{x}^{-1}x_{i},
\end{equation}
for any $x\in M$ as long as it is not in the cut locus of any of the data points. In particular, if $\{x_{i}\}_{i=1}^{N}\subset B(o,\rho)$, where $\rho<\frac{\textrm{inj}M}{2}$, then for any $x\in B(o,\rho)$ the above expression is well-defined in the classical sense (i.e., it is uniquely defined). Notice  that the above expression is well-defined for almost every $x\in M$ because the set at which $f_{p}$ is not differentiable has measure zero (for $p>1$ this set is $\cup_{i} \mathcal{C}_{x_{i}}$ and for $p=1$ it is $\cup_{i} \mathcal{C}_{x_{i}}\cup \{x_{i}\}_{i}$). As we will see this non-differentiability has severe implications on the behavior of the constant step-size gradient descent.

% Algorithm \ref{alg:rcm} is a gradient descent algorithm for locating the Riemannian center of mass of $\{x_{i}\}_{i=1}^{N}$.
% % todo
% \begin{figure}[h]
  % \centering
  % \begin{minipage}{1.\linewidth}
        \begin{algorithm}[H]
          % \caption{Compute Riemannian Center of Mass (RCM) on $(\gM, g)$}
        \caption{Compute RCM: Gradient Descent for finding the Riemannian $L^{p}$ center of mass of $\{x_{i}\}_{i=1}^{N}$}
          \label{alg:rcm}
            \begin{algorithmic}[1]
            \Require { $\{x_{i}\}_{i=1}^{N} \subset \gM$, $\{w_{i}\}_{i=1}^{N}$ and choose $x^{0}\in \gM$}
            % \State \emph{\# Compute $\bs{\mu}^{(i)}(t), \dot{\bs{\mu}}^{(i)}(t)$ using Eq. \ref{eq:posterior} and $\ddot{\b{z}}^{(i)}_\mesh$.}
            \State\label{algo:rcm:step1} \texttt{if} $\nabla f_{p}(x^{k})=0$ \texttt{then} stop, \texttt{else set}
              \begin{equation}\label{eq:rcm:gradient_descent}
              x^{k+1}=\exp_{x^{k}}(-t_{k}\nabla f_{p}(x^{k}))
              \end{equation}
              where $t_{k}>0$ is an ``appropriate'' step-size and $\nabla f_{p}(\cdot)$ is defined in (\ref{eq:grad_Lp}).
            \State \texttt{goto} step \ref{algo:rcm:step1}
            \end{algorithmic}
        \end{algorithm}
  % \end{minipage}
% \end{figure}

Besides practical considerations (e.g., stopping criterion), at least two important issues are left unspecified in Algorithm~\ref{alg:rcm}, namely, how to choose $x^{0}$ and how to choose $t_{k}$ for each $k$. The most natural choice for $x^{0}$ is one point in $B(o,\rho)$, say one of the data points. Note that in practice $o$ and the exact value of $\rho$ might not be known.





